Hierarchical Residual Attention Network for Single Image Super-Resolution

Convolutional neural networks are the most successful models in single image super-resolution. Deeper networks, residual connections, and attention mechanisms have further improved their performance. However, these strategies often improve the reconstruction performance at the expense of considerably increasing the computational cost. This paper introduces a new lightweight super-resolution model based on an efficient method for residual feature and attention aggregation. In order to make an efficient use of the residual features, these are hierarchically aggregated into feature banks for posterior usage at the network output. In parallel, a lightweight hierarchical attention mechanism extracts the most relevant features from the network into attention banks for improving the final output and preventing the information loss through the successive operations inside the network. Therefore, the processing is split into two independent paths of computation that can be simultaneously carried out, resulting in a highly efficient and effective model for reconstructing fine details on high-resolution images from their low-resolution counterparts. Our proposed architecture surpasses state-of-the-art performance in several datasets, while maintaining relatively low computation and memory footprint.

==> Draft.tex <==

% contains channel attention and a 1$\times$1 convolutional layer in order to aggregate and preserve the channel-wise features from all the channel attention layers for later use at the output of RAFG and the network. The channel attention inside the AB helps to efficiently extract the most important features from the whole channel-wise feature hierarchy. 




% Various attention mechanisms have been proposed in image SR. Although these methods contribute performance improvements, they impose additional limitations, starting with increases in computational cost. Moreover, most of them introduce a bottleneck layer to reduce the dimensionality of the features in order to speedup computation, but always at the cost of degrading channel information~\cite{wang2020eca}. 

% Let $\mathbf{r}_k$ be the output vector of the $k$-th residual block before element-wise addition inside the $k$-th RAFG. Then, the output of channel attention proceeds as:

% \begin{equation}
%     \mathbf{a}_k = CA(\mathbf{r}_k) ,
% \end{equation}
% where $\mathbf{a}_k$ is the output of the $k$-th Channel attention inside the $k$-th \resgroup. Each $\mathbf{a}_k$ is fed to the residual attention bank (\attentionbank) module which is composed of a channel attention and a $1\times$1 convolutional layer. The \attentionbank~is designed to to aggregate all the channel-wise features from all the channel attention layers. This attention-over-attention operation helps to efficiently extract the most important features from the whole feature hierarchy inside the k-$th$ \resgroup. Then the \attentionbank~proceed as:
% \begin{equation}
%     \mathbf{c}_k = CA(\operatorname{Conv}[a_o,...,a_k])
% \end{equation}
% where $[a_0,...,a_m]$ and CA denotes the outputs of each channel attention inside the k-$th$ \resgroup~and channel-wise attention operation respectively.  $\mathbf{c}_k$ represent the output of the \attentionbank which is used for later fusion at the end of the network. The final output of the k-$th$ \resgroup~can be presented as:
% \begin{equation}
%     \mathbf{o}_k = \mathbf{c}_k + \mathbf{a}_k + \textbf{x}_i
% \end{equation}
% where $\mathbf{O}_k$ represent the output of the k-$th$ \resgroup~and then is fed to the next \resgroup. 

% combines channel attention with residual blocks, but in contrast to other approaches, we propose to keep a dedicated computational path for attention modules, independent from the RFG path and parallel to it. Figure \ref{fig:main}~(bottom) shows that a RAFG contains three residual blocks, the output of which is respectively sent to a channel attention block. 
% Attention outputs are then globally aggregated by a bank of residual attentions, and the same happens with the features, which are globally combined by a bank of residual features. The attentional bank additionally incorporates an extra channel attention block, which helps to efficiently extract the most important components of the feature hierarchy. Finally, the outputs of both banks are combined together and sent to the subsequent RAFG.
%before element-wise addition are sent to the channel attention blocks and then concatenated together. We propose a residual attention feature bank (RAB) which contains channel attention and a 1$\times$1 convolutional layer in order to aggregate and preserve the channel-wise features from all the channel attention layers for later use at the output of RAFG and the network. The channel attention inside the RAB helps to efficiently extract the most important features from the whole channel-wise feature hierarchy. Finally, the outputs of RFB and RAB are combined together and sent to the next RAFG.


 
% 5555555555555555555555555555555555555555555555555555555555555555555555555555555555555
% Now, we give details about our proposed Feature-modulation bank module (RFB), outlined in the Figure \ref{}, which is composed of residual blocks (RBs), channel-wise attention module, hierarchical feature fusion (HFF) and channel-wise feature fusion (CAFF). 
% The extracted features by a deep network contain different types of information across channels. If we are able to increase the network's sensitivity to information-rich channels and make it focus on them, the representational power of the network would be enhanced and the performance improved. Keeping that in mind, we design a feature-modulation bank module (RFB), outlined in the Figure \ref{}, which is composed of residual blocks (RBs), channel-wise attention blocks (CAs), hierarchical feature fusion (HFF) and channe-wise feature fusion block (CAFF). The structure of the RFB is illustrated in Figure xx (). We detail each of these components below.\\
% \noindent \textbf{Channel-wise attention module}
% Various attention mechanisms have been proposed in the image SR. Although these methods improve the performance, they still have some limitations. Firstly, they often increase the computational cost. Secondly, most of the existing attention mechanisms introduce a bottleneck layer to reduce the dimensionality of the features in order to speedup computation at the cost of channel information degradation \cite{wang2020eca}. 

% To solve these problems, we design a channel-wise attention mechanism (CA) that improves the network performance without using bottleneck layers nor increasing the computational cost. The aim of the channel attention module is to recalibrates channel-wise feature responses by explicitly modeling interdependencies between channels. The structure of the channel attention is illustrated in Figure \ref{fig:rb_RFF}.  We denote U = [$u_1$, ..., $u_c$] as the input of the channel attention module, which consists of X feature maps with size of $H\timesW$. The c-th element of z is computed by 
% \begin{equation}
%     z_c = \frac{1}{H\times W}\sum_{i=1}^{H}\sum_{j=1}^{W}u_c(i,j),
% \end{equation}
% where $u_c=(i,j)$ is the value at position $(i,j)$ of the c-th channel $u_c$. To attend to the most relevant feature maps, we employ a gating mechanism with a sigmoid activation. the process is represented as follows:
% \begin{equation}
%     \alpha =\sigma (W_{LCA} * z),
% \end{equation}
% where $\sigma$ represents the sigmoid function, and  $*$ denotes the 1$\times$1 convolution operation.  $W_{LCA}$ is the weight of the convolutional layer. Then we obtain the final channel importance weights, which are used to rescale the input $u_c$
% \begin{equation}
%     \tilde{u}_c = z_c . u_c,
% \end{equation}

% where $z_c$ and $u_c$ are respectively the scaling factor and feature map in the c-th channel. With the above process, the channel attention is able to adaptively modulate the channel-wise features according to the channel-wise statistics of input, and help the network boost the channel-wise feature discriminative capacity without losing channel information.\\
% \noindent \textbf{Combining channel attention into the Residual Blocks.}
% Channel attention extracts the channel statistics among channels to further enhance the discriminative ability of the network. Previous approaches performed channel attention \textit{in-place} inside the residual blocks to further boost the representational ability of the network \cite{hu2018squeeze}. This usually implied an element-wise product between the attention output and the residual block output. However, this in-place channel attention may discard relevant details which will no longer be available in deeper levels of the neural architecture. To solve this issue, in contrast to previous approaches, we propose to move the attention modules outside of the main computational path of the network (see Figure \ref{fig:att}). Let $\textbf{x}_i$ and $\textbf{x}_o$ be the input and output vectors of the $k$-th RB inside the $d$-th RFB module. Then, the RB before element-wise addition proceeds as 
% \begin{equation}
%     \textbf{x}_o = \operatorname{Conv}(\delta(\operatorname{Conv}(\textbf{x}_{i}))),
% \end{equation}
% where $\delta$ denotes as the ReLU function. Then $\textbf{x}_o$ is fed to the attention module. Then we have
% \begin{equation}
%     \textbf{a}_o = CA(\textbf{x}_o) ,
% \end{equation}
% % \begin{equation}
% %     \textbf{x}_o = \textbf{x}_o + \textbf{x}_i,
% % \end{equation}
% where $\textbf{a}_o$ is the outputs of the $k$-th channel attention inside the $d$-th RFB. As a result, since attention is not directly applied to the residual block outputs, all the information is preserved, and attention outputs are concatenated for later use. \\
% \noindent \textbf{Integrating HFF and CAFF into the RFB.}
% Stacking residual blocks has been key to construct deep SISR networks \cite{lim2017enhanced}. However, depth comes with the cost of loss of information and training instability. Consider the residual blocks depicted in Figure \ref{fig:rb_RFF} (Left) introduced in the EDSR \cite{lim2017enhanced} and HAN \cite{niu2020single} architectures. Each time a set of features is passed through those blocks, lost information cannot be recovered and the longest the path it has to traverse the more information could be lost. Moreover, since these blocks are not aware of the computations performed by other blocks, they are limited to very local operations. 

% To solve these issues, we propose a hierarchical feature fusion module (HFF) to reduce low-level feature degradation and to boost the representation ability of the network. Figure \ref{fig:main} (Down) shows the details of a RFB which contains three residual blocks. All the outputs of the residual blocks are directly sent to the end of HRR block where they are concatenated with the input of the first residual block. However, these feature maps contain a large amount of redundant information. Moreover, using them directly in the next residual feature fusion block would greatly increase the computational complexity, since the amount of feature channels grows with each concatenation. In order to adaptively extract useful information from these hierarchical features, we introduce a bottleneck layer instantiated by a 1$\times$1 convolution. The output of these hierarchical features can be formulated as
% \begin{equation}
%     S_{RFB,d} = \operatorname{Conv_{1\times1}} ([f_0,...,F_{D-1}])
% \end{equation}
% where $F_{RFF}$ denotes the output of $k$-th RFB and $[f_0,...,F_{D-1}]$ refers to the concatenation of feature maps produced by residual RBs. 
% At the same time, we design a novel channel-wise feature fusion (CAFF) module to aggregate all the channel-wise features from all the channel attention layers.  This attention-over-attention operation helps to efficiently extract the most important features from the whole feature hierarchy. The final output of the CAFF can be presented as
% \begin{equation}
%     A_{CAFF,d} = CA(\operatorname{Conv_{1\times1}}([a_0,...,a_m]))) 
% \end{equation}
% where $[a_0,...,a_m]$ denotes the outputs of each channel attention inside the d-$th$ RFB and channel attention represent channel-wise attention operation. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Then $\textbf{x}_o$ is sent to the next residual block. The final output of the $k$-th residual feature fusion module is obtained as 
% \begin{equation}
%     \textbf{a}_o = LCA(\operatorname{Conv}[a^1_o,...,a^n_o])
% \end{equation}
% \begin{equation}
%     \textbf{x}_o = \operatorname{Conv}[x^1_o,...,x^n_o]).
% \end{equation}
% \noindent \textbf{Channel-wise Feature Fusion}

%It has been demonstrated that stacked residual blocks (RBs) can be used to construct deep networks in \cite{lim2017enhanced}. However, in image SR, very deep network built in such way would suffer from training difficulty and performance bottleneck due to the problem of gradient vanishing and exploding in deep networks.
%Moreover, the RB can generate useful hierarchical features focusing on different aspects of the original LR image. Figure \ref{fig:rb_RFF} (Left) depicts a basic residual block used in EDSR \cite{lim2017enhanced} and HAN \cite{niu2020single}. Consider the scenario of several consecutive residual blocks, the residual features of preceding blocks must go through a long path to propagate
%to subsequent blocks. Therefore, the residual feature information gradually disappears during the transmission and residual blocks play a very local role in the learning process of the whole network. 

% \noindent \textbf{Hierarchical Feature Fusion}


% where the per-channel summary statistics are calculated and then used to selectively emphasize informative feature-maps as well as suppress useless ones.

% \subsection{Deep Feature Extractor}
% We now give more details about our proposed deep feature extractor (see Figure \ref{fig:architecture}). The deep feature extractor computes useful representations of the LR patch in order to infer its HR version. Concretely, the deep feature extractor is based on residual-attention blocks which contains residual feature fusion modules and lightweight channel attention modules. We describe each of these below.
% % \begin{figure}[h]
% %     \centering
% %     \includegraphics[width=1\linewidth]{Figures/a.pdf}
% %     \captionsetup[figure]{font=small,skip=5pt}
% %     \caption{\textbf{Left}: A basic residual module. \textbf{Right}: Details of the RFF module, which contains three residual blocks (RB) and a 1$\times$1 convolutional layer. }
% %     \label{fig:rb_RFF}
% % \end{figure}
% \subsubsection{Residual feature fusion framework}
% It has been demonstrated that stacked residual blocks can be used to construct deep networks in \cite{lim2017enhanced}. However, in image SR, very deep network built in such way would suffer from training difficulty.
% % and performance bottleneck due to the problem of gradient vanishing and exploding in deep networks.
% Moreover, the residual blocks can generate useful hierarchical features focusing on different aspects of the original LR image. Figure \ref{fig:rb_RFF} (Left) depicts a basic residual block used in EDSR \cite{lim2017enhanced} and HAN \cite{niu2020single}. Consider the scenario of several consecutive residual blocks, the residual features of
% preceding blocks must go through a long path to propagate
% to subsequent blocks. Therefore, the residual feature information gradually disappears during the transmission and residual blocks play a very local role in the learning process of the whole network. 

% To solve these issues, we propose a residual feature fusion module to reduce low-level feature degradation and to boost the representation ability of the network. Figure \ref{fig:rb_RFF} (Right) shows the details of a residual feature fusion module which contains three residual blocks. All the outputs of the residual blocks are directly sent to the end of residual feature fusion block where they are concatenated with the input of the first residual block. On the one hand, these feature maps contain a large amount of redundant information. On the other hand, using them directly in the next residual feature fusion block will greatly increase the computational complexity, since the amount of feature channels grows with each concatenating. In order to adaptively extract useful information from these hierarchical features, we introduce a bottleneck layer which is a 1$\times$1 convolution. The output of these hierarchical features can be formulated as
% \begin{equation}
%     F_{RFF} = \operatorname{Conv_{1\times1}} ([f_0,...,F_{D-1}])
% \end{equation}
% where $F_{RFF}$ denotes the output of $k$-th residual feature fusion module and $[f_0,...,F_{D-1}]$ refers to the concatenation of feature maps produced by residual feature fusion modules. 

% \subsubsection{Lightweight channel attention}
% The extracted features by a deep network contain different types of information across channels. If we are able to increase the network's sensitivity to information-rich channels and make it focus on them, the representational power of the network would be enhanced and the performance improved. For this purpose, various channel attention mechanism have been proposed in image SR \cite{niu2020single,zhang2018image}. Although these methods improve the performance, they still have some limitations. Firstly, they often increase the computational cost. Secondly, most of the existing attention mechanisms introduce a bottleneck layer to reduce the dimensionality of the features in order to speedup computation at the cost of channel information degradation \cite{wang2020eca}.

% To solve these problems, we design a lightweight channel attention mechanism that improves the network performance without using bottleneck layers nor increasing the computational cost. 

% %without dimensionality reduction, which rather maintains channel information and in turn improves performance. 

% The structure of the lightweight channel attention is illustrated in Figure \ref{fig:rb_RFF}. We denote U = [$u_1$, ..., $u_c$] as the input of the lightweight channel attention module, which consists of X feature maps with size of $H\timesW$. The c-th elemant of z is computed by 
% \begin{equation}
%     z_c = \frac{1}{H\times W}\sum_{i=1}^{H}\sum_{j=1}^{W}u_c(i,j),
% \end{equation}
% where $u_c=(i,j)$ is the value at position $(i,j)$ of the c-th channel $u_c$. To assign different attentions to different types of feature maps, we employ a gating mechanism with a sigmoid activation to summary statistic z. the process is represented as follows:
% \begin{equation}
%     \alpha =\sigma (W_{LCA} * z),
% \end{equation}
% where $\sigma$ represents the sigmoid function, and  $*$ denotes the convolution operation. $W_{LCA}$ is the weight of the convolutional layer. Then we obtain the final channel statistics s, which is used to rescale the input $u_c$
% \begin{equation}
%     \tilde{u}_c = z_c . u_c
% \end{equation}

% where $z_c$ and $u_c$ are the scaling factor and feature map in the c-th channel. 

% With the above process, the Lchannel attention unit is able to adaptively modulate the channel-wise features according to the channel-wise statistics of input, and help the network boost the channel-wise feature discriminability without losing channel information.
% % \begin{figure}[h]
% %     \centering
% %     \includegraphics[width=1\linewidth]{Figures/Basic_residual.pdf}
% %     \includegraphics[width=1\linewidth]{Figures/residul_attention.pdf}
% %     \captionsetup[figure]{font=small,skip=5pt}
% %     \caption{\textbf{Left}: A basic residual module. \textbf{Right}: Details of the RFF module, which contains three residual blocks (RB) and a 1$\times$1 convolutional layer. }
% %     \label{fig:att}
% % \end{figure}
% \subsubsection{residual attention feature fusion module}
% As discussed above, residual feature fusion modules allow the low-level feature information to bypass the next computations inside the block and reach the output without suffering degradation. Channel attention extracts the channel statistics among channels to further enhance the discriminative ability of the network. Previous approaches combined channel attention into the residual blocks to further boost the representational ability of the network. This usually implied an element-wise product between the attention output and the residual block output. However, this \textit{in-place} channel attention may discard relevant details which will no longer be available in deeper levels of the neural architecture. To solve this issue, in contrast to previous approaches, we propose to move the attention modules outside of the main computational path of the network (see Figure \ref{fig:att}). Let $\textbf{x}_i$ and $\textbf{x}_o$ be the input and output vectors of the $k$-th residual block inside the $k$-th residual feature fusion module. Then, the residual block before element-wise addition proceeds as 
% \begin{equation}
%     \textbf{x}_o = \operatorname{Conv}(\delta(\operatorname{Conv}(\textbf{x}_{i}))),
% \end{equation}
% where $\delta$ denotes as the ReLU function. Then $\textbf{x}_o$ is fed to the attention module. Then we have
% \begin{equation}
%     \textbf{a}_o = LCA(\textbf{x}_o) ,
% \end{equation}
% \begin{equation}
%     \textbf{x}_o = \textbf{x}_o + \textbf{x}_i,
% \end{equation}
% where $\textbf{a}_o$ and $\textbf{x}_o$ are the outputs of the $k$-th attention and the $k$-th residual block inside the $k$-th residual feature fusion module. Then $\textbf{x}_o$ is sent to the next residual block. The final output of the $k$-th residual feature fusion module is obtained as 
% \begin{equation}
%     \textbf{a}_o = LCA(\operatorname{Conv}[a^1_o,...,a^n_o])
% \end{equation}
% \begin{equation}
%     \textbf{x}_o = \operatorname{Conv}[x^1_o,...,x^n_o]).
% \end{equation}

% % The output of residual feature fusion modules  are concatenate with channel attention feature maps at the end of the network. and propose a novel residual-attention fusion module. Therefore, residual fusion block and channel module are independent and executed in parallel. Let $\textbf{x}_i$ be the input vector of the $k$-th residual block inside the residual feature fusion module. Then, the residual block proceeds as 
% % \begin{equation}
% %     \textbf{x}_o = \operatorname{Conv}(\delta(\operatorname{Conv}(\textbf{x}_{i}))),
% % \end{equation}
% % where $\textbf{x}_o$ is the output vector of residual block before elemant-wise addition. Later,  $\textbf{x}_o$ is fed to the attention module and after elemant-wise addition to the next residual block. Then we can further have
% % \begin{equation}
% %      \textbf{a}_o = LCA(\textbf{x}_o)
% % \end{equation}
% % \begin{equation}
% %      \textbf{x}_o = \textbf{x}_o + \textbf{x}_{i}
% % \end{equation}
% % Later all output of attentions are concatenated and to reduce the dimensionality pass to the 1x1 convolution. To reweighting the attention we further use another LCA. So we have
% % \begin{equation}
% %      \textbf{x}_o = LCA(\operatorname{Conv}[a^1_o,...,a^n_o])
% % \end{equation}
% % This recursion is repeated for all residual-attention module within the main-blocks. In this way, we gather all local information and attentions progressively. 

% % To increase the network capacity, a similar recursion is applied  to  the  main-blocks. In order to facilitate access to local information,  the final output of the network receives the concatenation of the outputs of all the residual feature fusion modules and attentions. We combine the outputs off residual feature fusion with attention. 



% % \input{Tabels/local_global_attention}
% % \input{Tabels/Attentions}
% % \input{Tabels/in_out_attention_residual}
% % information is lost during the dimensionality reduction step in SE networks.












\section{Hierarchical Residual Attention Network}
\label{sec:proposed_method}
In this section, we first propose the overview of HARN network for SISR. Then we detail the proposed residual attention feature group (RAFG) and its components.

% each of the two main architectural patterns proposed in this paper: the so-called residual attention feature group and a novel lightweight channel attention module.

\subsection{Network Framework}
As shown in Figure~\ref{fig:main}, our proposed architecture (\architecture{}) consists of a non-linear mapping module and a final reconstruction block.
Let's denote  $I_{LR}$ and $I_{SR}$ as the input and output of \architecture, respectively. As recommended in \cite{ledig2017photo,lim2017enhanced}, we apply only one convolutional layer to extract the initial features $F_0$ from the LR input image
\begin{equation}
    F_{0}= \operatorname{Conv}(I_{LR}),
\end{equation}

Then the extracted feature $F_0$ is sent to the non-linear mapping module which compute useful representations of the LR patch in order to infer its HR version. We further introduce a long-range skip connection to grant access to the original information and facilitate the back-propagation of the gradients. The final output before the reconstruction step is then, 
\begin{equation}
    \mathcal{O} = F + F_0,
\end{equation}
where $F$ denotes the output of the non-linear mapping module. 

After acquiring the high informative features $\mathcal{O}$, we employ the sub-pixel convolutional layer \cite{shi2016real} as to upsample them:
\begin{equation}
    F_{\uparrow} = \mathcal{U} _{\uparrow}(\mathcal{O}) ,
\end{equation}
where $\mathcal{U}(.)$ and $\mathcal{U}$ are the upscale module and the upscaled features respectively. The upscaled features are then mapped into the SR image via one convolutional layer
\begin{equation}
    I_{SR} = D(X) = \mathcal{R} (F_{\uparrow}) ,
\end{equation}
where $\mathcal{R}(.)$, $\mathcal{R}$ denote the reconstruction layer, the upscale layer and the whole \architecture{} network respectively.\\
To verify the effectivness of our \architecture{}, we adopt the same loss function as previous works (\textit{e.g.,} $L_1$ loss function). Given a training set with $N$ LR images and their HR counterparts denoted by \{${I^{i}_{LR}, I^{i}_{HR}}$\}$^N_{i=1}$, the goal of training \architecture{} is to optimize the $L_1$ loss function:
\begin{equation}
  L(\Theta ) = \frac{1}{N} \sum_{N}^{i=1}\left \|D(X) -  I^{HR}\right\|_1,
\end{equation}
where $\theta$ denotes the parameter set of \architecture. 

\input{Tabels/RFG}
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.75\linewidth, height=3.3cm]{Figures/Channel_attention_residual.pdf}\par
    \captionsetup[figure]{font=small,skip=0pt}
    \caption{\small Proposed mechanism for extracting channel-wise attention from residual blocks.}
    \label{fig:attention}
\end{figure}
\subsection{Residual Attention Feature Group}
The residual attention feature group (RAFG) is designed to attend and preserve higher frequency details across the whole network. As shown in Figure~\ref{fig:main} (bottom), it is composed of two dedicated computational paths: feature extractor and channel attentions. We detail each of these below.\\
\indent\textbf{Feature extraction}. It has been demonstrated that stacked residual blocks facilitate the task of training deeper SISR networks. Figure~\ref{tab:RFG}~(a) depicts a common network design where consecutive residual blocks are stacked together to construct deep networks. In such designs, residual features from preceding residual blocks must go through a long path to propagate to subsequent residual blocks. Therefore, the residual feature information gradually disappears during the transmission and residual blocks play a very local role in the learning process of the whole network.  

To solve these issues, we propose a residual feature group (\resgroup) to reduce feature degradation and to boost the representation ability of the network. Figure \ref{tab:RFG}~(b) shows the details of a \resgroup~module which contains three residual blocks. The output of each residual block is linearly fused at the \resgroup~output in order to access to the hierarchical features. However, these hierarchical features contain a large amount of redundant information. Therefore, we propose to reduce the number of features at the end of each \resgroup. We name this feature aggregation and reduction step as feature bank. The reduction is done with a 1$\times$1 convolutional layer which suppresses the redundant features obtained by systematic feature concatenation. Compared with the way of simply stacking multiple residual blocks, our RFG enables non-local use of the residual features. The hierarchical information that preceding residual blocks contain can be propagated to the end of the RFG without any loss or interference, thus leading to a more discriminative feature representation. \\
\indent\textbf{Lightweight channel attention module}. To further improve the performance of \architecture~ we also propose a channel attention module, lightweight channel attention (LCA), improving performance with small increase in computational cost. Its structure is illustrated in Figure~\ref{fig:attention}. The attention recalibrates feature responses by implicitly modeling interdependencies between channels. In order to make it efficient, we propose to use a single 1x1 convolutional layer instead of the two 1x1 convolutional bottleneck commonly used in the literature \cite{zhang2018image}. Formally, we denote $U = [u_1, ..., u_c]$ as the input of the LCA module, which consists of $C$ feature maps $u_i$ of size $H\times W$. These feature maps are first reduced in the spatial dimensions by an average pooling operation,
\begin{equation}
    z_c = \frac{1}{H\times W}\sum_{i=1}^{H}\sum_{j=1}^{W}u_c(i,j),
\end{equation}
where $u_c(i,j)$ is the value at position $(i,j)$ of the $c$-th channel and $z_c$ is the resulting feature vector after average-pooling. To attend to the most relevant feature maps, we employ a gating mechanism with sigmoid activation:
\begin{equation}
    \alpha =\sigma (W_{LCA} * z),
\end{equation}
where $\sigma$ represents the sigmoid function, and  $*$ denotes a convolution operation by a $1\times1$ convolution kernel $W_{LCA}$. Then we obtain the final channel importance weights, which are used to rescale the input $u_c$

\begin{equation}
    \tilde{u}_c = z_c . u_c.
\end{equation}



\indent\textbf{Integrating LCA into Residual Blocks}. The features extracted by a deep network contain different types of information in each of the different channels. If we are able to increase the network's sensitivity to information-rich channels and make it focus on them, the efficiency of the network would be enhanced and the performance improved. In the literature, channel attention mechanism have been one of the most successful strategies for this purpose. Previous approaches performed channel attention \textit{in-place} inside the residual blocks to further boost the representational ability of the network \cite{hu2018squeeze}. This usually implied an element-wise product between the attention output and the residual block output. However, this in-place channel attention may discard relevant details which will no longer be available in deeper levels of the neural architecture.

To solve this issue, we propose an attention bank which combines LCA with residual blocks, but in contrast to other approaches, we propose to keep a dedicated computational path for attention modules, independent from the RFG path and parallel to it. Figure \ref{fig:main}~(bottom) shows that a RAFG contains three residual blocks, the output of which is respectively sent to a LCA block before element-wise addition. 
Attention outputs are then globally aggregated by a bank of attentions, and the same happens with the features, which are globally combined by a bank of features. The attention bank additionally incorporates an extra LCA block, which helps to efficiently extract the most important components of the feature hierarchy. Finally, the outputs of both banks are combined together and sent to the subsequent RAFG.

% contains channel attention and a 1$\times$1 convolutional layer in order to aggregate and preserve the channel-wise features from all the channel attention layers for later use at the output of RAFG and the network. The channel attention inside the AB helps to efficiently extract the most important features from the whole channel-wise feature hierarchy. 




% Various attention mechanisms have been proposed in image SR. Although these methods contribute performance improvements, they impose additional limitations, starting with increases in computational cost. Moreover, most of them introduce a bottleneck layer to reduce the dimensionality of the features in order to speedup computation, but always at the cost of degrading channel information~\cite{wang2020eca}. 

% Let $\mathbf{r}_k$ be the output vector of the $k$-th residual block before element-wise addition inside the $k$-th RAFG. Then, the output of channel attention proceeds as:

% \begin{equation}
%     \mathbf{a}_k = CA(\mathbf{r}_k) ,
% \end{equation}
% where $\mathbf{a}_k$ is the output of the $k$-th Channel attention inside the $k$-th \resgroup. Each $\mathbf{a}_k$ is fed to the residual attention bank (\attentionbank) module which is composed of a channel attention and a $1\times$1 convolutional layer. The \attentionbank~is designed to to aggregate all the channel-wise features from all the channel attention layers. This attention-over-attention operation helps to efficiently extract the most important features from the whole feature hierarchy inside the k-$th$ \resgroup. Then the \attentionbank~proceed as:
% \begin{equation}
%     \mathbf{c}_k = CA(\operatorname{Conv}[a_o,...,a_k])
% \end{equation}
% where $[a_0,...,a_m]$ and CA denotes the outputs of each channel attention inside the k-$th$ \resgroup~and channel-wise attention operation respectively.  $\mathbf{c}_k$ represent the output of the \attentionbank which is used for later fusion at the end of the network. The final output of the k-$th$ \resgroup~can be presented as:
% \begin{equation}
%     \mathbf{o}_k = \mathbf{c}_k + \mathbf{a}_k + \textbf{x}_i
% \end{equation}
% where $\mathbf{O}_k$ represent the output of the k-$th$ \resgroup~and then is fed to the next \resgroup. 

% combines channel attention with residual blocks, but in contrast to other approaches, we propose to keep a dedicated computational path for attention modules, independent from the RFG path and parallel to it. Figure \ref{fig:main}~(bottom) shows that a RAFG contains three residual blocks, the output of which is respectively sent to a channel attention block. 
% Attention outputs are then globally aggregated by a bank of residual attentions, and the same happens with the features, which are globally combined by a bank of residual features. The attentional bank additionally incorporates an extra channel attention block, which helps to efficiently extract the most important components of the feature hierarchy. Finally, the outputs of both banks are combined together and sent to the subsequent RAFG.
%before element-wise addition are sent to the channel attention blocks and then concatenated together. We propose a residual attention feature bank (RAB) which contains channel attention and a 1$\times$1 convolutional layer in order to aggregate and preserve the channel-wise features from all the channel attention layers for later use at the output of RAFG and the network. The channel attention inside the RAB helps to efficiently extract the most important features from the whole channel-wise feature hierarchy. Finally, the outputs of RFB and RAB are combined together and sent to the next RAFG.


 
% 5555555555555555555555555555555555555555555555555555555555555555555555555555555555555
% Now, we give details about our proposed Feature-modulation bank module (RFB), outlined in the Figure \ref{}, which is composed of residual blocks (RBs), channel-wise attention module, hierarchical feature fusion (HFF) and channel-wise feature fusion (CAFF). 
% The extracted features by a deep network contain different types of information across channels. If we are able to increase the network's sensitivity to information-rich channels and make it focus on them, the representational power of the network would be enhanced and the performance improved. Keeping that in mind, we design a feature-modulation bank module (RFB), outlined in the Figure \ref{}, which is composed of residual blocks (RBs), channel-wise attention blocks (CAs), hierarchical feature fusion (HFF) and channe-wise feature fusion block (CAFF). The structure of the RFB is illustrated in Figure xx (). We detail each of these components below.\\
% \noindent \textbf{Channel-wise attention module}
% Various attention mechanisms have been proposed in the image SR. Although these methods improve the performance, they still have some limitations. Firstly, they often increase the computational cost. Secondly, most of the existing attention mechanisms introduce a bottleneck layer to reduce the dimensionality of the features in order to speedup computation at the cost of channel information degradation \cite{wang2020eca}. 

% To solve these problems, we design a channel-wise attention mechanism (CA) that improves the network performance without using bottleneck layers nor increasing the computational cost. The aim of the channel attention module is to recalibrates channel-wise feature responses by explicitly modeling interdependencies between channels. The structure of the channel attention is illustrated in Figure \ref{fig:rb_RFF}.  We denote U = [$u_1$, ..., $u_c$] as the input of the channel attention module, which consists of X feature maps with size of $H\timesW$. The c-th element of z is computed by 
% \begin{equation}
%     z_c = \frac{1}{H\times W}\sum_{i=1}^{H}\sum_{j=1}^{W}u_c(i,j),
% \end{equation}
% where $u_c=(i,j)$ is the value at position $(i,j)$ of the c-th channel $u_c$. To attend to the most relevant feature maps, we employ a gating mechanism with a sigmoid activation. the process is represented as follows:
% \begin{equation}
%     \alpha =\sigma (W_{LCA} * z),
% \end{equation}
% where $\sigma$ represents the sigmoid function, and  $*$ denotes the 1$\times$1 convolution operation.  $W_{LCA}$ is the weight of the convolutional layer. Then we obtain the final channel importance weights, which are used to rescale the input $u_c$
% \begin{equation}
%     \tilde{u}_c = z_c . u_c,
% \end{equation}

% where $z_c$ and $u_c$ are respectively the scaling factor and feature map in the c-th channel. With the above process, the channel attention is able to adaptively modulate the channel-wise features according to the channel-wise statistics of input, and help the network boost the channel-wise feature discriminative capacity without losing channel information.\\
% \noindent \textbf{Combining channel attention into the Residual Blocks.}
% Channel attention extracts the channel statistics among channels to further enhance the discriminative ability of the network. Previous approaches performed channel attention \textit{in-place} inside the residual blocks to further boost the representational ability of the network \cite{hu2018squeeze}. This usually implied an element-wise product between the attention output and the residual block output. However, this in-place channel attention may discard relevant details which will no longer be available in deeper levels of the neural architecture. To solve this issue, in contrast to previous approaches, we propose to move the attention modules outside of the main computational path of the network (see Figure \ref{fig:att}). Let $\textbf{x}_i$ and $\textbf{x}_o$ be the input and output vectors of the $k$-th RB inside the $d$-th RFB module. Then, the RB before element-wise addition proceeds as 
% \begin{equation}
%     \textbf{x}_o = \operatorname{Conv}(\delta(\operatorname{Conv}(\textbf{x}_{i}))),
% \end{equation}
% where $\delta$ denotes as the ReLU function. Then $\textbf{x}_o$ is fed to the attention module. Then we have
% \begin{equation}
%     \textbf{a}_o = CA(\textbf{x}_o) ,
% \end{equation}
% % \begin{equation}
% %     \textbf{x}_o = \textbf{x}_o + \textbf{x}_i,
% % \end{equation}
% where $\textbf{a}_o$ is the outputs of the $k$-th channel attention inside the $d$-th RFB. As a result, since attention is not directly applied to the residual block outputs, all the information is preserved, and attention outputs are concatenated for later use. \\
% \noindent \textbf{Integrating HFF and CAFF into the RFB.}
% Stacking residual blocks has been key to construct deep SISR networks \cite{lim2017enhanced}. However, depth comes with the cost of loss of information and training instability. Consider the residual blocks depicted in Figure \ref{fig:rb_RFF} (Left) introduced in the EDSR \cite{lim2017enhanced} and HAN \cite{niu2020single} architectures. Each time a set of features is passed through those blocks, lost information cannot be recovered and the longest the path it has to traverse the more information could be lost. Moreover, since these blocks are not aware of the computations performed by other blocks, they are limited to very local operations. 

% To solve these issues, we propose a hierarchical feature fusion module (HFF) to reduce low-level feature degradation and to boost the representation ability of the network. Figure \ref{fig:main} (Down) shows the details of a RFB which contains three residual blocks. All the outputs of the residual blocks are directly sent to the end of HRR block where they are concatenated with the input of the first residual block. However, these feature maps contain a large amount of redundant information. Moreover, using them directly in the next residual feature fusion block would greatly increase the computational complexity, since the amount of feature channels grows with each concatenation. In order to adaptively extract useful information from these hierarchical features, we introduce a bottleneck layer instantiated by a 1$\times$1 convolution. The output of these hierarchical features can be formulated as
% \begin{equation}
%     S_{RFB,d} = \operatorname{Conv_{1\times1}} ([f_0,...,F_{D-1}])
% \end{equation}
% where $F_{RFF}$ denotes the output of $k$-th RFB and $[f_0,...,F_{D-1}]$ refers to the concatenation of feature maps produced by residual RBs. 
% At the same time, we design a novel channel-wise feature fusion (CAFF) module to aggregate all the channel-wise features from all the channel attention layers.  This attention-over-attention operation helps to efficiently extract the most important features from the whole feature hierarchy. The final output of the CAFF can be presented as
% \begin{equation}
%     A_{CAFF,d} = CA(\operatorname{Conv_{1\times1}}([a_0,...,a_m]))) 
% \end{equation}
% where $[a_0,...,a_m]$ denotes the outputs of each channel attention inside the d-$th$ RFB and channel attention represent channel-wise attention operation. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Then $\textbf{x}_o$ is sent to the next residual block. The final output of the $k$-th residual feature fusion module is obtained as 
% \begin{equation}
%     \textbf{a}_o = LCA(\operatorname{Conv}[a^1_o,...,a^n_o])
% \end{equation}
% \begin{equation}
%     \textbf{x}_o = \operatorname{Conv}[x^1_o,...,x^n_o]).
% \end{equation}
% \noindent \textbf{Channel-wise Feature Fusion}

%It has been demonstrated that stacked residual blocks (RBs) can be used to construct deep networks in \cite{lim2017enhanced}. However, in image SR, very deep network built in such way would suffer from training difficulty and performance bottleneck due to the problem of gradient vanishing and exploding in deep networks.
%Moreover, the RB can generate useful hierarchical features focusing on different aspects of the original LR image. Figure \ref{fig:rb_RFF} (Left) depicts a basic residual block used in EDSR \cite{lim2017enhanced} and HAN \cite{niu2020single}. Consider the scenario of several consecutive residual blocks, the residual features of preceding blocks must go through a long path to propagate
%to subsequent blocks. Therefore, the residual feature information gradually disappears during the transmission and residual blocks play a very local role in the learning process of the whole network. 

% \noindent \textbf{Hierarchical Feature Fusion}


% where the per-channel summary statistics are calculated and then used to selectively emphasize informative feature-maps as well as suppress useless ones.

% \subsection{Deep Feature Extractor}
% We now give more details about our proposed deep feature extractor (see Figure \ref{fig:architecture}). The deep feature extractor computes useful representations of the LR patch in order to infer its HR version. Concretely, the deep feature extractor is based on residual-attention blocks which contains residual feature fusion modules and lightweight channel attention modules. We describe each of these below.
% % \begin{figure}[h]
% %     \centering
% %     \includegraphics[width=1\linewidth]{Figures/a.pdf}
% %     \captionsetup[figure]{font=small,skip=5pt}
% %     \caption{\textbf{Left}: A basic residual module. \textbf{Right}: Details of the RFF module, which contains three residual blocks (RB) and a 1$\times$1 convolutional layer. }
% %     \label{fig:rb_RFF}
% % \end{figure}
% \subsubsection{Residual feature fusion framework}
% It has been demonstrated that stacked residual blocks can be used to construct deep networks in \cite{lim2017enhanced}. However, in image SR, very deep network built in such way would suffer from training difficulty.
% % and performance bottleneck due to the problem of gradient vanishing and exploding in deep networks.
% Moreover, the residual blocks can generate useful hierarchical features focusing on different aspects of the original LR image. Figure \ref{fig:rb_RFF} (Left) depicts a basic residual block used in EDSR \cite{lim2017enhanced} and HAN \cite{niu2020single}. Consider the scenario of several consecutive residual blocks, the residual features of
% preceding blocks must go through a long path to propagate
% to subsequent blocks. Therefore, the residual feature information gradually disappears during the transmission and residual blocks play a very local role in the learning process of the whole network. 

% To solve these issues, we propose a residual feature fusion module to reduce low-level feature degradation and to boost the representation ability of the network. Figure \ref{fig:rb_RFF} (Right) shows the details of a residual feature fusion module which contains three residual blocks. All the outputs of the residual blocks are directly sent to the end of residual feature fusion block where they are concatenated with the input of the first residual block. On the one hand, these feature maps contain a large amount of redundant information. On the other hand, using them directly in the next residual feature fusion block will greatly increase the computational complexity, since the amount of feature channels grows with each concatenating. In order to adaptively extract useful information from these hierarchical features, we introduce a bottleneck layer which is a 1$\times$1 convolution. The output of these hierarchical features can be formulated as
% \begin{equation}
%     F_{RFF} = \operatorname{Conv_{1\times1}} ([f_0,...,F_{D-1}])
% \end{equation}
% where $F_{RFF}$ denotes the output of $k$-th residual feature fusion module and $[f_0,...,F_{D-1}]$ refers to the concatenation of feature maps produced by residual feature fusion modules. 

% \subsubsection{Lightweight channel attention}
% The extracted features by a deep network contain different types of information across channels. If we are able to increase the network's sensitivity to information-rich channels and make it focus on them, the representational power of the network would be enhanced and the performance improved. For this purpose, various channel attention mechanism have been proposed in image SR \cite{niu2020single,zhang2018image}. Although these methods improve the performance, they still have some limitations. Firstly, they often increase the computational cost. Secondly, most of the existing attention mechanisms introduce a bottleneck layer to reduce the dimensionality of the features in order to speedup computation at the cost of channel information degradation \cite{wang2020eca}.

% To solve these problems, we design a lightweight channel attention mechanism that improves the network performance without using bottleneck layers nor increasing the computational cost. 

% %without dimensionality reduction, which rather maintains channel information and in turn improves performance. 

% The structure of the lightweight channel attention is illustrated in Figure \ref{fig:rb_RFF}. We denote U = [$u_1$, ..., $u_c$] as the input of the lightweight channel attention module, which consists of X feature maps with size of $H\timesW$. The c-th elemant of z is computed by 
% \begin{equation}
%     z_c = \frac{1}{H\times W}\sum_{i=1}^{H}\sum_{j=1}^{W}u_c(i,j),
% \end{equation}
% where $u_c=(i,j)$ is the value at position $(i,j)$ of the c-th channel $u_c$. To assign different attentions to different types of feature maps, we employ a gating mechanism with a sigmoid activation to summary statistic z. the process is represented as follows:
% \begin{equation}
%     \alpha =\sigma (W_{LCA} * z),
% \end{equation}
% where $\sigma$ represents the sigmoid function, and  $*$ denotes the convolution operation. $W_{LCA}$ is the weight of the convolutional layer. Then we obtain the final channel statistics s, which is used to rescale the input $u_c$
% \begin{equation}
%     \tilde{u}_c = z_c . u_c
% \end{equation}

% where $z_c$ and $u_c$ are the scaling factor and feature map in the c-th channel. 

% With the above process, the Lchannel attention unit is able to adaptively modulate the channel-wise features according to the channel-wise statistics of input, and help the network boost the channel-wise feature discriminability without losing channel information.
% % \begin{figure}[h]
% %     \centering
% %     \includegraphics[width=1\linewidth]{Figures/Basic_residual.pdf}
% %     \includegraphics[width=1\linewidth]{Figures/residul_attention.pdf}
% %     \captionsetup[figure]{font=small,skip=5pt}
% %     \caption{\textbf{Left}: A basic residual module. \textbf{Right}: Details of the RFF module, which contains three residual blocks (RB) and a 1$\times$1 convolutional layer. }
% %     \label{fig:att}
% % \end{figure}
% \subsubsection{residual attention feature fusion module}
% As discussed above, residual feature fusion modules allow the low-level feature information to bypass the next computations inside the block and reach the output without suffering degradation. Channel attention extracts the channel statistics among channels to further enhance the discriminative ability of the network. Previous approaches combined channel attention into the residual blocks to further boost the representational ability of the network. This usually implied an element-wise product between the attention output and the residual block output. However, this \textit{in-place} channel attention may discard relevant details which will no longer be available in deeper levels of the neural architecture. To solve this issue, in contrast to previous approaches, we propose to move the attention modules outside of the main computational path of the network (see Figure \ref{fig:att}). Let $\textbf{x}_i$ and $\textbf{x}_o$ be the input and output vectors of the $k$-th residual block inside the $k$-th residual feature fusion module. Then, the residual block before element-wise addition proceeds as 
% \begin{equation}
%     \textbf{x}_o = \operatorname{Conv}(\delta(\operatorname{Conv}(\textbf{x}_{i}))),
% \end{equation}
% where $\delta$ denotes as the ReLU function. Then $\textbf{x}_o$ is fed to the attention module. Then we have
% \begin{equation}
%     \textbf{a}_o = LCA(\textbf{x}_o) ,
% \end{equation}
% \begin{equation}
%     \textbf{x}_o = \textbf{x}_o + \textbf{x}_i,
% \end{equation}
% where $\textbf{a}_o$ and $\textbf{x}_o$ are the outputs of the $k$-th attention and the $k$-th residual block inside the $k$-th residual feature fusion module. Then $\textbf{x}_o$ is sent to the next residual block. The final output of the $k$-th residual feature fusion module is obtained as 
% \begin{equation}
%     \textbf{a}_o = LCA(\operatorname{Conv}[a^1_o,...,a^n_o])
% \end{equation}
% \begin{equation}
%     \textbf{x}_o = \operatorname{Conv}[x^1_o,...,x^n_o]).
% \end{equation}

% % The output of residual feature fusion modules  are concatenate with channel attention feature maps at the end of the network. and propose a novel residual-attention fusion module. Therefore, residual fusion block and channel module are independent and executed in parallel. Let $\textbf{x}_i$ be the input vector of the $k$-th residual block inside the residual feature fusion module. Then, the residual block proceeds as 
% % \begin{equation}
% %     \textbf{x}_o = \operatorname{Conv}(\delta(\operatorname{Conv}(\textbf{x}_{i}))),
% % \end{equation}
% % where $\textbf{x}_o$ is the output vector of residual block before elemant-wise addition. Later,  $\textbf{x}_o$ is fed to the attention module and after elemant-wise addition to the next residual block. Then we can further have
% % \begin{equation}
% %      \textbf{a}_o = LCA(\textbf{x}_o)
% % \end{equation}
% % \begin{equation}
% %      \textbf{x}_o = \textbf{x}_o + \textbf{x}_{i}
% % \end{equation}
% % Later all output of attentions are concatenated and to reduce the dimensionality pass to the 1x1 convolution. To reweighting the attention we further use another LCA. So we have
% % \begin{equation}
% %      \textbf{x}_o = LCA(\operatorname{Conv}[a^1_o,...,a^n_o])
% % \end{equation}
% % This recursion is repeated for all residual-attention module within the main-blocks. In this way, we gather all local information and attentions progressively. 

% % To increase the network capacity, a similar recursion is applied  to  the  main-blocks. In order to facilitate access to local information,  the final output of the network receives the concatenation of the outputs of all the residual feature fusion modules and attentions. We combine the outputs off residual feature fusion with attention. 



% % \input{Tabels/local_global_attention}
% % \input{Tabels/Attentions}
% % \input{Tabels/in_out_attention_residual}
% % information is lost during the dimensionality reduction step in SE networks.











==> Tabels/AB.tex <==
\begin{table}[!h]
\centering
\footnotesize
\caption{\small Effects of attention bank (AB) inside and outside of the RFG Urban100 with $\times$4. The best result is \textbf{highlighted}.}
\setlength\arrayrulewidth{0.3pt}

\begin{tabular}{c@{~~~}|c@{~~~~~~~~~}c@{~~~~~~~~~}c@{~~~~~~~~~}c@{~~~~~~}}
% \cline{2-5}
\toprule
\multicolumn{1}{c|}{\textbf{Config}} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4}\\
\midrule
AB in RFG &$\times$&\checkmark&$\times$& \checkmark\\
AB out RFG &$\times$&$\times$&\checkmark& \checkmark\\\hline
PSNR & 26.24 & 26.32 & 26.29 & \textbf{26.39}\\\bottomrule

\end{tabular}

\label{tab:AB}
\end{table}
